Bootstrapping Tensor Integrals

This work proposes a bootstrapping with positivity methodology to study random $U(N)^{D}$ invariant tensors in the large $N$ limit. As has been done for $U(N)$ invariant random matrices, we combine the Dyson-Schwinger equations and positivity constraints of moments to approximate the moments of such tensor models. As examples, we bootstrap the quartic and two hexic rank three tensor models. All models studied converge quickly, and for those which have known analytic formulae, they converge to such solutions. We conjecture new explicit formulae for all moments of the rank three quartic model and support this conjecture using bootstrapped results and explicit double-series computations with 'feyntensor'.

==> kbordermatrix.tex <==
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{kbordermatrix}[2011/09/21 Bordered matrix with brackets]

%	Author:	Kim C Border <kcborder@caltech.edu>
%	Date:		SuperBowl XXXVII (Go Bucs)

%   Revised 2003/09/20
%		to allow flush right option.
%   Revised 2011/09/21 
%		at urging of Bruno Calfa (CMU) 
%		to coexist with package arydshln
%		by adding \def\@xarraycr ... 

%	Defines \kbordermatrix along the lines of plain tex's
%	\bordermatrix (which is still available in LaTeX).

%	In particular, as with \bordermatrix,
%	1.	It takes the array as an argument.  It does not use \begin{}..\end{}.
%		Is this a feature or a bug?
%	2.	The first row is spaced a bit further apart from the rest.
%	3.	The lower (n-1) by (n-1) block is set off by delimiters.
%	4.	There is an invisible bottom row of the same height as the segregated
%		top row that adds to the height of the equation.

%	Differences from \bordermatrix:
%	1.  Square brackets are used in place of parentheses.
%	2.  You may use \\ instead of \cr.
%	3.  The line heights agree with LaTeX's line heights for the
%		array environment, and \arraystretch is respected.  This means
%		the bottom (n-1) rows align with the rows of an (n-1)-rowed
%		\begin{array}..\end{array} (with or without delimiters).
%	4.	All columns are centered.
%	** Modified 2003-9-20 to allow flush right option.
%	5.	The first column is spaced a bit further apart from the rest.


%	Differences from \left\[\begin{array}...\end{array}\right\]
%	1.	It takes the array as an argument.  It does not use \begin{}..\end{}.
%		Is this a feature or a bug?
%	2.	Consequently, you cannot use a column specifier (e.g., {l|cr}).
%	3.	Consequently the maximum number of columns is not specified.
%	4.	Vertical rules must be put in each row in a separate column.
%	5.  You can use \hline and \cline.

%	At least it works in the cases I have tried, but I offer no guarantees.



%	cf. \bordermatrix p. 361, and \vrulealign p. 392 of The TeXbook



%	Style parameters, they may be redefined according to taste.
	\newcommand{\kbldelim}{[}	%	Left delimiter
	\newcommand{\kbrdelim}{]}%	Right delimiter
			
	\newcommand{\kbrowstyle}{\scriptstyle}%  Style applied to first row
	\newcommand{\kbcolstyle}{\scriptstyle}%   Style applied to first column
	
	\newlength{\kbcolsep}		%	Extra separation after first border column
	\newlength{\kbrowsep}		%	Extra separation after first border row
	
	\setlength{\kbcolsep}{.5\arraycolsep}
	\setlength{\kbrowsep}{.2ex}
	
	\newif\ifkbalignright

%	Scratch lengths (to be computed)
	\newlength{\br@kwd}		%	Width of delimiter
	\newlength{\k@bordht}	%	Height of border column 
	
%	This is it
\newcommand{\kbordermatrix}[1]{%
\begingroup
  	%	\br@kwd depends on font size, so compute it now.
	\setbox0=\hbox{$\left\kbldelim\right.$}
	\setlength{\br@kwd}{\wd0}
		%	Compute the array strut based on current value of \arraystretch.
	\setbox\@arstrutbox\hbox{\vrule 
		\@height\arraystretch\ht\strutbox 	
		\@depth\arraystretch\dp\strutbox
		\@width\z@}
		%	Compute height of first row and extra space.
	\setlength{\k@bordht}{\kbrowsep}
	\addtolength{\k@bordht}{\ht\@arstrutbox}
	\addtolength{\k@bordht}{\dp\@arstrutbox}
		%	turn off mathsurround
	\m@th
		%	Set the first row style
	\def\@kbrowstyle{\kbrowstyle}
		%	Swallow the alignment into box0:
	\setbox0=\vbox{%
			%	Define \cr for first row to include the \kbrowsep
			%	and to reset the row style
		\def\cr{\crcr\noalign{\kern\kbrowsep
			\global\let\cr=\endline
			\global\let\@kbrowstyle=\relax}}
			%	Redefine \\ a la LaTeX:
		\let\\\@arraycr
			%	The following are needed to make a solid \vrule with no gaps
			%	between the lines.
		\lineskip\z@skip	
		\baselineskip\z@skip	
			%	Compute the length of the skip after the first column
		\dimen0\kbcolsep \advance\dimen0\br@kwd
			%	Here begins the alignment:
		\ialign{\tabskip\dimen0		%	This space will show up after the first column
			\kern\arraycolsep\hfil\@arstrut$\kbcolstyle ##$\hfil\kern\arraycolsep&
			\tabskip\z@skip			%	Cancel extra space for other columns
			\kern\arraycolsep\hfil$\@kbrowstyle ##$\ifkbalignright\relax\else\hfil\fi\kern\arraycolsep&&
			\kern\arraycolsep\hfil$\@kbrowstyle ##$\ifkbalignright\relax\else\hfil\fi\kern\arraycolsep\crcr
				%	That ends the template.
				%	Here is the argument:
			#1\crcr}%		End \ialign
	}%	End \setbox0.
		%	\box0 now holds the array.
		%
		%	This next line uses \box2 to hold a throwaway 
		%	copy of \box0, leaving \box0 intact,
		%	while putting the last row in \box5.
	\setbox2=\vbox{\unvcopy0 \global\setbox5=\lastbox}
		%	We want the width of the first column,
		%	so we lop off columns until there is only one left.
		%	It's not elegant or efficient, but at 1 gHz, who cares.
	\loop
		\setbox2=\hbox{\unhbox5 \unskip \global\setbox3=\lastbox}
		\ifhbox3
			\global\setbox5=\box2
			\global\setbox1=\box3
	\repeat
		%	\box1 now holds the first column of last row.
		%
		%	This next line stores the alignment in \box2, 
		%	while calculating the proper
		%	delimiter height and placement.
	\setbox2=\hbox{$\kern\wd1\kern\kbcolsep\kern-\arraycolsep
		\left\kbldelim
		\kern-\wd1\kern-\kbcolsep\kern-\br@kwd
			%
			%	Here is the output.  The \vcenter aligns the array with the "math axis."
			%	The negative vertical \kern only shrinks the delimiter's height.
			%	BTW, I didn't find this in the TeXbook, 
			%	I had to try various \kerns to see what they did in a 
			%	\left[\vcenter{}\right].
	\vcenter{\kern-\k@bordht\vbox{\unvbox0}}
	\right\kbrdelim$}
	\null\vbox{\kern\k@bordht\box2}
		%
	\endgroup
}


